Generalized Multiple Correlation Coefficient as a Similarity Measurements between Trajectories

Similarity distance measure between two trajectories is an essential tool to understand patterns in motion, for example, in Human-Robot Interaction or Imitation Learning. The problem has been faced in many fields, from Signal Processing, Probabilistic Theory field, Topology field or Statistics field.Anyway, up to now, none of the trajectory similarity measurements metrics are invariant to all possible linear transformation of the trajectories (rotation, scaling, reflection, shear mapping or squeeze mapping). Also not all of them are robust in front of noisy signals or fast enough for real-time trajectory classification. To overcome this limitation this paper proposes a similarity distance metric that will remain invariant in front of any possible linear transformation.Based on Pearson Correlation Coefficient and the Coefficient of Determination, our similarity metric, the Generalized Multiple Correlation Coefficient (GMCC) is presented like the natural extension of the Multiple Correlation Coefficient. The motivation of this paper is two fold. First, to introduce a new correlation metric that presents the best properties to compute similarities between trajectories invariant to linear transformations and compare it with some state of the art similarity distances.Second, to present a natural way of integrating the similarity metric in an Imitation Learning scenario for clustering robot trajectories.

==> References.tex <==
for analyses of interactions between multiple persons
with early adoption by the computer vision community (Oliver et al., 2000). More recently, HMMs have
been proposed in several works related to human-robot
interaction. Lee et al. (2010) used a hierarchical HMM
to learn and represent robot behaviors. In their approach, a high-level HMM identifies the current state
of the interaction and triggers low-level HMMs which
correspond to the robot’s motor primitives. To ensure
that the robot adapts to the movement of the human
partner, virtual springs were attached between markers on the human body and corresponding positions
on the robot. Tanaka et al. (2012) proposed a Markov
model to predict the positions of a worker in an assembly line. The space in which the worker moves is
discretized into different regions and a Gaussian mixture model was used to relate positions to procedures.
Using this information a robot could then deliver tools
and parts to a human worker along the assembly line.
More recently, a path-map HMM approach was used
to model interactions in cooperative tasks in which a
backbone of shared hidden states correlates the actions
of the interacting agents (Ben Amor et al., 2013).
Besides HMMs, other probabilistic graphical models have also been used to address interaction tasks.
Koppula and Saxena (2013) used an augmented Conditional Random Field where the additional nodes and
edges of the graph are used to capture sub-activities,
human poses, object affordances and object locations
over time. Inference on the graphical model, allows a
robot to anticipate the human activity. In a separate
step, a pre-programmed robot response is selected accordingly such that it can help the human in achieving
the recognized task. In contrast to our work, the output
of our method is a movement primitive that is intrinsically correlated to the human action and can be used to
directly control the robot. Wang et al. (2013) proposed
an intention-driven dynamics model to encode human
intentions as latent states in a graphical model. Intentions can be modeled as discrete variables, such as action labels, or continuous variables, such as an object’s







\subsection{Applied GMCC for Human-Robot interaction}\label{GMCC3}

For a complete collaboration between humans and robots, improving robot's adaptation to unknown is important. In front of an unknown human command, the robots should be able to generalize and interpret the command in similarity relation to previously received commands. GMCC similarity distance metric from equation \ref{distance} can be a very useful tool for this task. GMCC can generalize the human command to any linear transformation, it will deal with noise and it has a fast response.

Considering an already known human commands library, when a new human command arrives, the robot will compute the similarity of this new command with the commands in the library and classify. 














An important approach to the intuition and finding patterns in the data had been done by the statistician Karl Pearson in the late 19th century. Pearson's correlation coefficient, also known as product-moment correlation coefficient is a measure that will measure how dependant two scalar random variables X and Y. The Pearson's correlation coefficient

$$\rho = \frac{Cov(X,Y)}{\sqrt{\sigma_x^2\sigma_y^2}}$$
will be 0 if X and Y are mutually independent. In case, there is a linear correlation between the random variables X and Y, then the Pearson's correlation coefficient will measure the strength of that correlation.

Pearson's correlation is limited to univariate variables. In the case of univariate dependant variable y and multiple independent variables $X = (x_1,x_2,\dots,x_n)$, the multiple correlation coefficient is considered as the extension of the Pearson's correlation and a particular case of the coefficient of determination. 

The correlation coefficients diverges when multidimensional random variables are considered for both dependant and independent variables. One of the first methods to compute the correlation of two multivariate random variables had been proposed by Harold Hotelling in 1936. The Canonical Correlation Coefficient(CCA) measure the correlation and the vectors a,b such that the correlation between $a^TX$ and $b^TY$ is maximized

$$(a^*,b^*) = argmax_{a,b}\rho(a^TX,b^TY) $$

Another solution was proposed by Y. Escoufier in 1973. The RV coefficient also know as $\rhoV$ coefficient is a correlation coefficient for multidimensional random variables X and Y. Escoufier's metric was a big advantage in comparison with CCA as the correlation coefficient remains rotation and scale invariance.


==> bibliography.tex <==
\bibitem{dc}Sokal, R. R., & Rohlf, F. J. (n.d.). Introduction to Biostatistic, 2nd ed., pg.277, Ed. DOVER PUBLICATIONS, INC. Mineola, New York. 1969
\bibitem{mc}Neter, John, Michael H. Kutner, Christopher Nachtsheim, and William Wasserman.  Applied Linear Statistical Models.  McGraw Hill, Boston.  1996
\bibitem{EDR}Chen, Lei and Ozsu, M Tamer and Oria, Vincent. Robust and Fast Similarity Search for Moving Object Trajectories. 2005
\bibitem{TWED}Pierre-François Marteau. Time Warp Edit Distance. arXiv. 2008
\bibitem{imit}Takayuki Osa, Joni Pajarinen, Gerhard Neumann, J. Andrew Bagnell, Pieter Abbeel and Jan Peters (2018), "An Algorithmic Perspective on Imitation Learning", Foundations and Trends® in Robotics: Vol. 7: No. 1-2, pp 1-179.
\bibitem{imit2}Schaal, Stefan. "Learning from demonstration." Advances in neural information processing systems. 1997.
\bibitem{lanini1}Lanini, Jessica, et al. "Human Intention Detection as a Multiclass Classification Problem: Application in Physical Human–Robot Interaction While Walking." IEEE Robotics and Automation Letters 3.4 (2018): 4171-4178.
\bibitem{predict1}Oriane Dermy, Alexandros Paraschos, Marco Ewerton, Jan Peters, François Charpillet, et al.. Prediction of Intention during Interaction with iCub with Probabilistic Movement Primitives. Frontiers in Robotics and AI, Frontiers Media S.A., 2017, 4
\bibitem{general1}Amor, Heni Ben, et al. "Generalization of human grasping for multi-fingered robot hands." 2012 IEEE/RSJ International Conference on Intelligent Robots and Systems. IEEE, 2012.
\bibitem{mime}D. Lee, C. Ott, and Y. Nakamura, “Mimetic communication model with compliant physical contact in human-humanoid interaction,” The International Journal of Robotics Research, vol. 29, no. 13, pp. 1684– 1704, 2010
\bibitem{amor1}Amor, Heni Ben, et al. "Learning responsive robot behavior by imitation." 2013 IEEE/RSJ International Conference on Intelligent Robots and Systems. IEEE, 2013.
\bibitem{maeda1}Maeda, Guilherme, et al. "Learning interaction for collaborative tasks with probabilistic movement primitives." 2014 IEEE-RAS International Conference on Humanoid Robots. IEEE, 2014.
\bibitem{amor2}Amor, Heni Ben, et al. "Interaction primitives for human-robot cooperation tasks." 2014 IEEE international conference on robotics and automation (ICRA). IEEE, 2014.
\bibitem{parachos1}Paraschos, Alexandros, et al. "Probabilistic movement primitives." Advances in neural information processing systems. 2013.
\bibitem{gomez1}Gomez-Gonzalez, Sebastian, et al. "Adaptation and Robust Learning of Probabilistic Movement Primitives." arXiv preprint arXiv:1808.10648 (2018).
\bibitem{dtw1}Salvador, Stan, and Philip Chan. "Toward accurate dynamic time warping in linear time and space." Intelligent Data Analysis 11.5 (2007): 561-580.
\bibitem{EDR}Chen, Lei, M. Tamer Özsu, and Vincent Oria. "Robust and fast similarity search for moving object trajectories." Proceedings of the 2005 ACM SIGMOD international conference on Management of data. ACM, 2005.
\bibitem{ERP}Chen, Lei, and Raymond Ng. "On the marriage of lp-norms and edit distance." Proceedings of the Thirtieth international conference on Very large data bases-Volume 30. VLDB Endowment, 2004.
\bibitem{LCSS}Vlachos, Michail, Dimitrios Gunopoulos, and George Kollios. "Discovering similar multidimensional trajectories." icde. IEEE, 2002.
\bibitem{Frechet}Eiter, Thomas, and Heikki Mannila. Computing discrete Fréchet distance. Tech. Report CD-TR 94/64, Information Systems Department, Technical University of Vienna, 1994.
\bibitem{hausdorff}Henrikson, Jeff. "Completeness and total boundedness of the Hausdorff metric." MIT Undergraduate Journal of Mathematics 1 (1999): 69-80
\bibitem{hotelling1}Hotelling, Harold. "Relations between two sets of variates." Breakthroughs in statistics. Springer, New York, NY, 1992. 162-190.
\bibitem{escoufier1}Escoufier, Yves. "Le traitement des variables vectorielles." Biometrics (1973): 751-760.
\bibitem{escoufier2}Robert, Paul, and Yves Escoufier. "A unifying tool for linear multivariate statistical methods: the RV‐coefficient." Journal of the Royal Statistical Society: Series C (Applied Statistics) 25.3 (1976): 257-265.
\bibitem{dcov}Székely, Gábor J., and Maria L. Rizzo. "Brownian distance covariance." The annals of applied statistics 3.4 (2009): 1236-1265.
\bibitem{dcor}Székely, Gábor J., Maria L. Rizzo, and Nail K. Bakirov. "Measuring and testing dependence by correlation of distances." The annals of statistics 35.6 (2007): 2769-2794.
\bibitem{HRI_survey}Goodrich, Michael A., and Alan C. Schultz. "Human–robot interaction: a survey." Foundations and Trends® in Human–Computer Interaction 1.3 (2008): 203-275.
\bibitem{t_shi}Wang, Xiaoyan, et al. "Hidden-markov-models-based dynamic hand gesture recognition." Mathematical Problems in Engineering 2012 (2012).



